METRO: A Software-Hardware Co-Design of Interconnections for Spatial DNN Accelerators

Tiled spatial architectures have proved to be an effective solution to build large-scale DNN accelerators. In particular, interconnections between tiles are critical for high performance in these tile-based architectures. In this work, we identify the inefficiency of the widely used traditional on-chip networks and the opportunity of software-hardware co-design. We propose METRO with the basic idea of decoupling the traffic scheduling policies from hardware fabrics and moving them to the software level. METRO contains two modules working in synergy: METRO software scheduling framework to coordinate the traffics and METRO hardware facilities to deliver the data based on software configurations. We evaluate the co-design using different flit sizes for synthetic study, illustrating its effectiveness under various hardware resource constraints, in addition to a wide range of DNN models selected from real-world workloads. The results show that METRO achieves 56.3% communication speedup on average and up to 73.6% overall processing time reduction compared with traditional on-chip network designs.

==> asplos23-templates/sections/evaluation/syn-breakdown.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[htb]
\centering
\label{tab:cadence}
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{|ccccc|}
\hline
\multicolumn{2}{|c|}{\textbf{Modules}}               & \multicolumn{1}{c|}{\textbf{Parameter}} & \multicolumn{1}{c|}{\textbf{Area (mm$^2
\ $)}} & \textbf{Power (mW)} \\ \hline \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Router}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Register\\ File\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}5Kb input registers\\ 300 bits lookup table\end{tabular}} &
  \multicolumn{1}{c|}{0.02} &
  73.15 \\ \cline{2-5} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{Control} & \multicolumn{1}{c|}{1024 bit width}                  & \multicolumn{1}{c|}{0.08}                & 8.47               \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Core}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}MAC Array\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}$256 \times 8$-bit integer\end{tabular}} &
  \multicolumn{1}{c|}{2.34} &
  143.36 \\ \cline{2-5} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{Buffer}   & \multicolumn{1}{c|}{280KB SRAM}         & \multicolumn{1}{c|}{3.4}                & 28.91              \\ \hline \hline
\multicolumn{5}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}router area: 0.11 mm$^2\ $, router power: 81.62mW\\ core area: 5.74 mm$^2\ $, core power: 172.17mW\end{tabular}}} \\ \hline
\end{tabular}%
}
\caption{METRO area and power breakdown}
\label{tab:ppa_breakdown}
\end{table}

==> asplos23-templates/sections/introduction/introduction.tex <==
\section{Introduction}

Spatial architectures are demonstrated as a popular solution to build a large-scale, high-performance and elastic processing system for tensor applications, such as auto-pilot, recommendation systems, and complex system simulation. The state-of-art f

A typical spatial architecture integrates massive homogeneous processing elements (~PEs~) via an interconnection subsystem. 
% A tensor application, which is represented as a graph of tensor operators, flows through the PE array, and drives processing elements to perform different computation operations on data elements. These computation operations are pre-configured by compilers to processing elements based on their physical locations. 
% in a \textbf{spatial computing paradigm}: the tensor operators are pre-configured to the PEs by compilers, and input data flows through the PE array
Such architecture has a substantial advantage of scaling out performance  and
recent industrial efforts on TOPs-level accelerators demonstrate this trend: Simba has 576 PEs that provides 32~TOPs computation throughput~\cite{simba}; Graphcore IPU integrates 1472 PEs with over 8000 parallel threads~\cite{graphcore}; Cerebras even implements a spatial architecture on the wafer scale, accommodating up to 400,000 cores~\cite{cerebras}. 

As more and more processing elements are integrated in the spatial architecture, the interconnection becomes a critical design factor to fully utilize their computing capacity. The interconnection should ensure sufficient data fed to a PE to match the PE's computation throughput. Otherwise, the PE's computing cycles are wasted due to waiting the data to arrive. 

\wz{Previous assumes a NoC to provide a non-blocking data delivering between processing elements, but few researches are conducted on how to design it.}

Unfortunately, designing an efficient interconnection that enables high PE utilization is not travail. A straightforward interconnection design is to adapt a traditional network-on-chip~(NoC) architecture~\cite{tangram, simba, graphcore}. A typical traditional NoC comprises multiple routers connected with channels, and delivers data in a fixed-size packet. To schedule the data efficiently and reduce hardware complexity, comprehensive research projects have been proposed on routing algorithms, flow control mechanisms, and router micro-architectures. Fundamentally, these works deliver data via the so called ``hardware scheduling'' paradigm, which relies on hardware components embedded in routers to provide two functionalities: 
(1) \textit{path routing} to select a path from the source router to the destination router, on a given topology. 
(2) \textit{flow controlling} to resolve that multiple packets at a router desire the same output channel, typically resulting in allocating the channel to one packet and blocking the others. 

However, the hardware scheduling is constrained by latency and complexity of circuit. Limited by router's area, power, and frequency, hardware scheduling strategies are typically greedy or short-sighted. These strategies select the best solution available at the decision making moment, but being unaware of global traffic load. As a consequence, the hardware scheduling exhibits two problems: 
% For example, as a router is only aware of its neighbours, adaptive routing~\cite{mad} based on the one-hop buffer. 
% Although traditional NoCs have been comprehensively researched and been widely adopted in existing spatial architectures, we observe that their channels are seriously under-utilized. It fails to address the two aforementioned challenges. 
% This greedy feature results in serious low channel utilization, even when the traffic is heavy. 

\noindent First, the \textbf{tree path convergence} problem: 
the greedy hardware scheduling strategies generate the same multicast tree for various multicast packets. When processing a tensor application, spatial architectures usually takes a ``dataflow'' scheme to run a tensor operator on multiple processing elements. A dataflow splits a tensor operator into multiple sub-operators on some specific tensor dimensions, and executes these sub-operators with different processing elements. These processing elements share the operands, and induces multicast packets to deliver them. Hardware scheduling takes a tree-like path to send a multicast packet to its destinations, and forks the packets once reaching the tree branching points. However, the tree is formed based on the fixed priorities, and results various multicast trees converges to a same one.~\cite{one_to_m}

% First, processing a tensor involves intensive one-to-many ( multicast ) packets to distribute data from the source to the worker processing elements. These packets 
% Tree-based multicast
% Although multicast packets are different in sources and destinations, the greedy routing algorithm selects similar paths for them. 
\noindent Second, the \textbf{sparse congestion} problem: when some parts of the NoC have serious congestion, the other parts are under-utilized. A tensor application typically comprises multiple tensor operator categories, such as convolution and matrix-matrix multiplication. As these tensor operator categories have different computing intensities, they always require for different data feeding speeds, i.e. interconnection bandwidths.~\cite{heterogeneous, maestro, tenet, timeloop} For example, an element in a $3 \times 3$ convolution is computed xxx times than in a matrix multiplication; the convolution requires xxx higher bandwidth than the matrix multiplication does. As a consequence, the interconnection need to handle heterogeneous bandwidth throughout the array, as these tensor operators are mapped to different locations~\cite{multi_nn}. The heterogeneous bandwidth requirements results in unbalanced use of interconnection channels. 

% Second, tensor operators always require for different data feeding speeds, i.e. interconnection bandwidths, because of their different computing intensities. 
% while some channels are overloaded, the rest channels are under-utilized; the hardware scheduling fails to balance the traffic load globally. 
% However, designing an efficient interconnection subsystem to fit tensor applications is non-travail in two aspects: 
% First, processing a tensor involves intensive collective communication traffics, such as one-to-many ( multicast ) and many-to-one ( reduce ), to move data between processing elements; these traffics are very likely to cause hotspots, which substantially lead to congestion, tree-saturation and even deadlocks. Therefore, to deliver data in time, the interconnection should be smart enough to address these issues efficiently. 

% This constraint make hardware scheduling fails to address the two aforementioned traffic challenges. 
% When face the collective communication traffic, traditional NoCs meet the \textbf{path convergence} problem: collective communication patterns with different sources and destinations take over the same paths; the hardware scheduling fails to find divergent forwarding paths for them. 
% When face unbalanced bandwidth requirements, traditional NoCs suffer with the \textbf{sparse congestion} problem: while some channels are overloaded, the rest channels are under-utilized; the hardware scheduling fails to balance the traffic load globally. 


% Second, hardware routing is unable to re-balance the traffic globally~\cite{ppin, mad, romm}, which results in the ``sparse congestion'' problem. 

% but it's impossible for designers to develop a dedicated heterogeneous interconnection suitable for all cases. % 应该提到dynamic heterogeneous

% Therefore, different parts of the interconnection ought to provide different bandwidth, 
% Additionally, multiple tensor applications may be processed at the same time in scenarios, such as autonomous driving~\cite{autodrive} and cloud service~\cite{multi_nn}. 

% To fully utilize the massive processing elements, existing spatial architectures~\cite{eyeriss, shidiannao, nvdla, eyerissv2, tenstorrent, sambanova, cerebras, tangram, graphcore, simba} typically adopt a spatial computing paradigm: 

% A straightforward interconnection design is to adopt a traditional network-on-chip~(NoC) architecture~\cite{tangram, simba, graphcore} , with over-provision hardware resources, e.g. link width and router buffer, to account for the largest bandwidth requirement. A typical traditional NoC comprises multiple routers and delivers data in packets via the channels between them. In traditional NoCs, traffics are scheduled \textbf{distributively} by routers. Specifically, multiple functional hardware components are embedded in routers, accounting for different stages of traffic scheduling: when a packet receives a router, the router checks its routing table to determine the packet's output channels, queries its arbitrator to allocate buffer and channels, and maintains its credit controller to detect and manage down-streaming buffers. In this work, we collaboratively term this scheduling scheme as ``hardware scheduling''. 

To overcome the drawbacks of traditional NoCs, we propose to remove the traffic scheduling from the critical path of data delivering, and move it \textbf{entirely} to the software level. The rationale is that as tensor applications are mainly composed of deterministic tensor operations, we thus can acquire entire traffic information at application compiling phase. Based on this information, the software scheduler is able to instrument the collective communication traffic and balance the load globally. The benefits of software scheduling are two-folded. 
First, software has more time, and more traffic information, to find better scheduling policies than hardware scheduling does.
Second, after offloading the traffic control to software, the hardware design of NoC can be significantly simplified. This is attractive because the traditional NoC consumes substantial latency, energy, and area of a spatial architecture~\cite{simba, rethink_noc}. 

However, there are two key problems to adopt the idea of software scheduling. 
First, the software scheduling lacks a unified problem definition to work on: traffic scheduling in traditional NoCs comprises various stages, including multicast tree-generation, path routing and resource arbitration. In traditional NoC's working flow, these stages have been handled independently, with different problem formulations, different optimization algorithms, and different objectives. 
% Therefore, \wz{therefore what ? }.
Second, the software's scheduling results can be extremely large, taking substantial control overheads. The resulting scheduling contains routes and flow control information for each packet, and it's overhead scales linearly with the application and array size. 
% Therefore, the raw scheduling information takes considerable bits. 

To address the two challenges, we propose a holistic software scheduling framework called \name. We call it \name~because the metro traffic, which is well scheduled before an operation, has a similar deterministic feature. The drivers do not need to worry about traffic control during operation. \name~addresses two key problems to adopt the idea of software scheduling. 
% \textit{How to build a unified search space and objective for scheduling engines to work on? } Second, the resulting scheduling information can be extremely long. \textit{How to embed the information to minimize hardware control overheads? }
The main contributions of this work are summarized as follows, 

\begin{itemize}

\item We observe the ``sparse congestion'' and the ``path convergence'' problems when traditional NoCs processing tensor applications. 

\item By leveraging the prior knowledge of communication, we propose a win-win solution to offload the traffic scheduling policies to the software level. It not only mitigates the ``sparse congestion'' and the ``path convergence'' problems, but also reduces the hardware design complexity significantly. 

\item To unify the different optimization problems within traffic scheduling, we propose xxx, a unified problem definition of collective communication tree generation, routing and resource arbitration. And based on this abstraction, we provide a detailed design of the software traffic scheduler. 

% We provide a detailed design of the software traffic scheduler, which includes a dual-phase flow transformation, a global routing optimization, and a conflict-free flow control mechanism. 

\item To reduce scheduling information overhead, we further present lightweight NoC hardware cooperating with the software traffic scheduler. 
% Moreover, we propose to use a chunk granularity packet to reduce the traffic overhead. and a chunk granularity packet 

\item We develop a cycle-accurate simulation to evaluate the performance of our holistic solution (called \name) with widely-used tensor applications. We also provide energy and area results of lightweight hardware using commercial IC design tools. Experimental results prove the advantages of \name, in respect of performance, energy consumption, and chip area.

\end{itemize}


==> asplos23-templates/sections/methodology/discuss.tex <==

A straightforward way to co-design the architecture is to adopt the switch-based routers. Since the software arranges the routes and timing for all packets, routers can perform a static switching with only a single register at every input channels. There is no flow control mechanisms such as backpressure between routers to solve the blocking issues. However, a real-world tensor application can induce a small portion of dynamic traffic loads. The dynamic traffic refers to the packets whose issue time can not be accurately estimated before execution. The reasons of dynamic traffic has multiple folds, including DRAM bank conflicts, circuit controlling signals, etc. Consequently, for these packets, the \textit{Blocking Time Shift} technique can not guarantee conflict-free at the software level. In turn, the architecture should have the ability to solve the blocking issues. 

==> asplos23-templates/sections/methodology/overview.tex <==
\section{\name~Overview}

Starting from the idea of software traffic scheduling, we develop an software hardware co-design, named \name, to automatically search the scheduling space, evaluate the resulting strategies, and verify the hardware designs. \name~comprises a software scheduling framework and a co-designed lightweight hardware router. 

% \name~is compatible with existing compiling frameworks for tensor applications, and supports a wide range of hardware setups. 
% In this section, we first illustrate the definition of traffic scheduling problem and hardware setups, then we introduce the entire workflow.
% One of the design goal of \name~is to widely support existing works, including the workflows to compile tensor applications and spatial computing core designs. 



==> asplos23-templates/sections/related_work/related_work.tex <==
\section{Related Works}

\subsection{Oblivious Routing}

\subsection{Reconfigurable Architectures}
To achieve optimal communication throughput on different applications, some works reconfigured their interconnection topology to adapt to traffic features.~\cite{maeri, rethink_noc, eyerissv2} Their router connectivity is configured ahead of execution and maintains static during execution. However, their reconfigurability is achieved at the cost of high hardware overheads. The reconfigurable architectures typically reserve redundant routers and links at hardware and tailor them to form different typologies. The tailored substrates consume static energy and chip area but don't provide any bandwidth, while \name leverages every channel as much as possible. Consequently, \name can achieve the same performance as reconfigurable architectures do, but with much less energy consumption and a smaller chip area.

\subsection{Software Defined NoC}

Recent works on Software-Defined Network on Chip~\cite{sdnoc_survey, sdnoc_1} tried to balance the traffic by integrating a centralized monitor into the interconnection sub-system. The monitor collects global traffic information and adjusts run-time traffic scheduling policies. However, the approach cannot work with large-scale spatial architectures because the extra delay for controlling packet transmission increases rapidly with the number of PEs~\cite{sdnoc_survey}. \name removes the traffic scheduling from the router's critical path; our approach is more practical for large-scale spatial architectures as it does not induce additional delay in packet delivering. 

